Instant Payments After a Betting Ban: Evidence from Brazil

Brazil has been facing major problems with delinquency, household debt, high interest rates, consumption, and access to credit, while online sports betting has emerged in public debate as a possible contributing factor, culminating with the federal government banned betting nationwide On September 25, 2026. We compare the number and total value of instant payments Pix over the following 37 days with forecasts based on pre-ban data, finding that both outcomes were below forecast in all three models. Under the two quadratic-trend models, the number of transactions was 3.75-4.12% below forecast and total transaction value was about 3.68% below forecast, while the linear-trend model gave larger gaps of 8.37% and 10.83%, respectively. These gaps offer indirect evidence on the scale of Pix flows potentially linked to betting.

==> supplement_rows.tex <==
\newcommand{\PlaceboRows}{
Transaction count & S1 & All & -8.37 & 84 & 2 & 2.38 & -7.62 & -3.68 & 4.33 \\
Transaction count & S1 & Recent & -8.37 & 24 & 0 & 0.00 & -5.24 & -4.39 & -2.88 \\
Transaction count & S2 & All & -4.12 & 84 & 3 & 3.57 & -4.87 & 1.30 & 16.03 \\
Transaction count & S2 & Recent & -4.12 & 24 & 0 & 0.00 & -1.38 & 0.21 & 2.56 \\
Transaction count & S3 & All & -3.75 & 84 & 4 & 4.76 & -5.70 & 1.45 & 14.08 \\
Transaction count & S3 & Recent & -3.75 & 24 & 0 & 0.00 & -1.63 & 0.32 & 2.79 \\
Settlement value & S1 & All & -10.83 & 84 & 3 & 3.57 & -12.69 & -3.74 & 5.30 \\
Settlement value & S1 & Recent & -10.83 & 24 & 0 & 0.00 & -6.65 & -4.73 & -0.71 \\
Settlement value & S2 & All & -3.68 & 84 & 7 & 8.33 & -5.51 & 3.02 & 19.66 \\
Settlement value & S2 & Recent & -3.68 & 24 & 0 & 0.00 & -1.11 & 0.20 & 5.19 \\
Settlement value & S3 & All & -3.68 & 84 & 8 & 9.52 & -5.48 & 3.00 & 19.11 \\
Settlement value & S3 & Recent & -3.68 & 24 & 0 & 0.00 & -1.17 & 0.22 & 5.25 \\
}
\newcommand{\ValidationRows}{
Transaction count & S1 & Earlier & 60 & 3.88 & 3.24 \\
Transaction count & S1 & Recent & 24 & 4.49 & 4.49 \\
Transaction count & S1 & All & 84 & 4.05 & 3.60 \\
Transaction count & S2 & Earlier & 60 & 4.18 & -2.85 \\
Transaction count & S2 & Recent & 24 & 0.94 & -0.24 \\
Transaction count & S2 & All & 84 & 3.25 & -2.10 \\
Transaction count & S3 & Earlier & 60 & 4.20 & -2.89 \\
Transaction count & S3 & Recent & 24 & 1.05 & -0.36 \\
Transaction count & S3 & All & 84 & 3.30 & -2.17 \\
Settlement value & S1 & Earlier & 60 & 5.02 & 3.70 \\
Settlement value & S1 & Recent & 24 & 4.64 & 4.60 \\
Settlement value & S1 & All & 84 & 4.91 & 3.96 \\
Settlement value & S2 & Earlier & 60 & 6.80 & -2.94 \\
Settlement value & S2 & Recent & 24 & 1.18 & -0.63 \\
Settlement value & S2 & All & 84 & 5.20 & -2.28 \\
Settlement value & S3 & Earlier & 60 & 6.63 & -2.98 \\
Settlement value & S3 & Recent & 24 & 1.20 & -0.64 \\
Settlement value & S3 & All & 84 & 5.08 & -2.31 \\
}

